Testing Java implementations of algebraic specifications

In this paper we focus on exploiting a specification and the structures that satisfy it, to obtain a means of comparing implemented and expected behaviours and find the origin of faults in implementations. We present an approach to the creation of tests that are based on those specification-compliant structures, and to the interpretation of those tests' results leading to the discovery of the method responsible for an eventual test failure. Results of comparative experiments with a tool implementing this approach are presented.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{A. Petrenko, H. Schlingloff (Eds.): Eighth Workshop on\\ Model-Based Testing (MBT 2013)\\
EPTCS 111, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.111.4}{10.4204/EPTCS.111.4}}
\pdfoutput=1

